Performance Analysis and Approximate Message Passing Detection of Orthogonal Time Sequency Multiplexing Modulation

In orthogonal time sequency multiplexing (OTSM) modulation, the information symbols are conveyed in the delay-sequency domain upon exploiting the inverse Walsh Hadamard transform (IWHT). It has been shown that OTSM is capable of attaining a bit error ratio (BER) similar to that of orthogonal time-frequency space (OTFS) modulation at a lower complexity, since the saving of multiplication operations in the IWHT. Hence we provide its BER performance analysis and characterize its detection complexity. We commence by deriving its generalized input-output relationship and its unconditional pairwise error probability (UPEP). Then, its BER upper bound is derived in closed form under both ideal and imperfect channel estimation conditions, which is shown to be tight at moderate to high signal-to-noise ratios (SNRs). Moreover, a novel approximate message passing (AMP) aided OTSM detection framework is proposed. Specifically, to circumvent the high residual BER of the conventional AMP detector, we proposed a vector AMP-based expectation-maximization (VAMP-EM) detector for performing joint data detection and noise variance estimation. The variance auto-tuning algorithm based on the EM algorithm is designed for the VAMP-EM detector to further improve the convergence performance. The simulation results illustrate that the VAMP-EM detector is capable of striking an attractive BER vs. complexity trade-off than the state-of-the-art schemes as well as providing a better convergence. Finally, we propose AMP and VAMP-EM turbo receivers for low-density parity-check (LDPC)-coded OTSM systems. It is demonstrated that our proposed VAMP-EM turbo receiver is capable of providing both BER and convergence performance improvements over the conventional AMP solution.

==> acronyms.tex <==
%
%acronyms

\newacronym{AWGN}{AWGN}{additive white Gaussian noise}

\newacronym{BABF}{BABF}{blind adaptive beamforming}

\newacronym{BER}{BER}{bit error ratio}

\newacronym{CW}{CW}{continuous wave}

\newacronym{CU}{CU}{control unit}

\newacronym{JML}{JML}{joint maximum-likelihood}

\newacronym{DPSK}{DPSK}{differential phase shift key}

\newacronym{PSK}{PSK}{phase shift key}

\newacronym{EM}{EM}{expectation maximization}

\newacronym{PDF}{PDF}{probability density function}

\newacronym{CSI}{CSI}{channel state information}

\newacronym{EPC}{EPC}{electronic product code}

\newacronym{RF}{RF}{radio frequency}

\newacronym{RIP}{RIP}{rotational invariance property}

\newacronym{RFID}{RFID}{radio frequency identification}

\newacronym{IC}{IC}{integrated circuit}

\newacronym{IoTs}{IoTs}{Internet of Things}

\newacronym{ULA}{ULA}{uniform linear array}

\newacronym{UHF}{UHF}{ultra high frequency}

\newacronym{OLS}{OLS}{ordinary least square}

\newacronym{QCQPs}{QCQPs}{quadratically constrained quadratic programs}

\newacronym{SDR}{SDR}{semidefinite relaxation}

\newacronym{SCA}{SCA}{successive convex approximation}

\newacronym{WET}{WET}{wireless energy transfer}

\newacronym{UWB}{UWB}{ultrawide bandwidth}

\newacronym{ToA}{ToA}{time-of-arrival}

\newacronym{PoA}{PoA}{phase-of-arrival}

\newacronym{DoA}{DoA}{direction-of-arrival}

\newacronym{RSS}{RSS}{received signal strength}

\newacronym{MSE}{MSE}{mean square error}

\newacronym{DoF}{DoF}{degree of freedom}

\newacronym{UAV}{UAV}{unmanned aerial vehicle}

\newacronym{CAMs}{CAMs}{cooperative awareness messages}

\newacronym{BS}{BS}{base station}

\newacronym{ID}{ID}{identification}

\newacronym{PL}{PL}{platoon leader}

\newacronym{PM}{PM}{platoon member}
\newacronym{PMs}{PMs}{platoon members}

\newacronym{a.k.a.}{a.k.a.}{also know as}

\newacronym{DPM}{DPM}{disconnected platoon member}

\newacronym{BaS}{BaS}{Braking and Stopping}

\newacronym{TAs}{TAs}{transmit antennas}

\newacronym{RAs}{RAs}{receive antennas}

\newacronym{3D}{3D}{three-dimensional}

\newacronym{ACK}{ACK}{acknowledgement}

\newacronym{V2V}{V2V}{vehicle-to-vehicle}

\newacronym{V2I}{V2I}{vehicle-to-infrastructure}

\newacronym{WLAN}{WLAN}{wireless local area network}

\newacronym{UAVs}{UAVs}{unmanned aerial vehicles}

\newacronym{ML}{ML}{machine learning}

\newacronym{TOA}{TOA}{time of arrival}

\newacronym{UWB}{UWB}{ultrawideband}

\newacronym{OBU}{OBU}{on-board unit}

\newacronym{LOS}{LOS}{line-of-sight}

\newacronym{RIB}{RIB}{rotational invariance beamforming}




















